Multiagent Finetuning: Self Improvement with Diverse Reasoning Chains

Large language models (LLMs) have achieved remarkable performance in recent years but are fundamentally limited by the underlying training data. To improve models beyond the training data, recent works have explored how LLMs can be used to generate synthetic data for autonomous self-improvement. However, successive steps of self-improvement can reach a point of diminishing returns. In this work, we propose a complementary approach towards self-improvement where finetuning is applied to a multiagent society of language models. A group of language models, all starting from the same base model, are independently specialized by updating each one using data generated through multiagent interactions among the models. By training each model on independent sets of data, we illustrate how this approach enables specialization across models and diversification over the set of models. As a result, our overall system is able to preserve diverse reasoning chains and autonomously improve over many more rounds of fine-tuning than single-agent self-improvement methods. We quantitatively illustrate the efficacy of the approach across a wide suite of reasoning tasks.

==> figText/likelihoods.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/likelihoods-iters-ft.pdf}
    \vspace{-10pt}
    \caption{\textcolor{blue}{\textbf{Measuring response likelihood of other agents across iterations of finetuning.} We measure the response diversity using likelihood of generated responses from other agents using a held-out agent across iterations of finetuning. We see that the diversity increases via an increase in NLL across iteration of finetuning for our method. }}
    \label{fig:enter-label}
    \vspace{-15pt}
\end{figure}

==> figText/mean_consensus-iters.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/likelihoods-iters-ft.pdf}
    \vspace{-10pt}
    \caption{\textcolor{red}{\textbf{TODO: Vighnesh is making this plot for mistral}}\small \textbf{Response diversity across finetuning iterations}. We measure the response diversity of our method and the single-agent finetuning method on the MATH dataset. The diversity of our method remains consistent over finetuning iterations, whereas the diversity of the single-agent method drops significantly.}
    \label{fig:mean_con}
    \vspace{-15pt}
\end{figure}


% \begin{figure}
% \centering
% \begin{tikzpicture}
%     \node[anchor=south west, inner sep=0] (image1) at (0,0) {\includegraphics[width=0.6\textwidth]{rebuttal/embed_diss-iters-ft.pdf}};
%     \node[anchor=south west, inner sep=0] (image2) at (0.6\textwidth,0) {\includegraphics[width=0.33\textwidth]{rebuttal/scatter_sim_acc-1.pdf}};
    
%     \node[anchor=north west, inner sep=2pt, font=\bfseries] at ([yshift=9pt]image1.north west) {(a)};
%     \node[anchor=north west, inner sep=2pt, font=\bfseries] at ([yshift=9pt]image2.north west) {(b)};
% \end{tikzpicture}
% \caption{\textcolor{red}{\bf VS: Will split this figure}. \small \textbf{Response diversity across finetuning iterations}. We measure the response diversity of our method and the single-agent finetuning method on the MATH dataset. (a) The diversity of our method remains consistent over finetuning iterations, whereas the diversity of the single-agent method drops significantly. (b) We compare accuracy of over rounds of finetuning with our embedding dissimilarity metric. We find that accuracy improves as diversity increases.}
% \label{fig:mean_con}
% \vspace{-10pt}
% \end{figure}

==> figText/teaser.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/new_teaser_figure.pdf}
    \vspace{-20pt}\caption{\textbf{Mutliagent finetuning improves reasoning performance}. 
    Our multiagent finetuning method, whether applied to open-source language models such as Mistral or proprietary models like GPT-3.5, significantly outperforms the original models on three reasoning tasks.}
    \label{fig:teaser}
    \vspace{-5pt}
\end{figure}
